On the Structure of Abstract H*-Algebras

Previously we have shown that the topos approach to quantum theory of Doering and Isham can be generalised to a class of categories typically studied within the monoidal approach to quantum theory of Abramsky and Coecke. In the monoidal approach to quantum theory H*-algebras provide an axiomatisation of states and observables. Here we show that H*-algebras naturally correspond with the notions of states and observables in the generalised topos approach to quantum theory. We then combine these results with the dagger-kernel approach to quantum logic of Heunen and Jacobs, which we use to prove a structure theorem for H*-algebras. This structure theorem is a generalisation of the structure theorem of Ambrose for H*-algebras the category of Hilbert spaces.

==> eptcsdata.tex <==
\providecommand{\firstpage}{197}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.13}{10.4204/EPTCS.266.13}}

